Meta-F*: Proof Automation with SMT, Tactics, and Metaprograms

We introduce Meta-F*, a tactics and metaprogramming framework for the F* program verifier. The main novelty of Meta-F* is allowing the use of tactics and metaprogramming to discharge assertions not solvable by SMT, or to just simplify them into well-behaved SMT fragments. Plus, Meta-F* can be used to generate verified code automatically. Meta-F* is implemented as an F* effect, which, given the powerful effect system of F*, heavily increases code reuse and even enables the lightweight verification of metaprograms. Metaprograms can be either interpreted, or compiled to efficient native code that can be dynamically loaded into the F* type-checker and can interoperate with interpreted code. Evaluation on realistic case studies shows that Meta-F* provides substantial gains in proof development, efficiency, and robustness.

==> interop_lazy/cor.tex <==
\begin{corollary}[F* native tactic compilation correctness] \ \\
  If
  \begin{itemize}
  \item $\hastyp{\cdot}{\cdot}{\sval}{\sarrow{\staui}{\stauii}}$
  \item $\hastyp{\cdot}{\svar{x} : \sarrow{\staui}{\stauii}}{\sexpp}{\stau}$
  \item $\sval \trans \tval$
  \end{itemize}
  then
  $\rexp{\stau}{\sexpp\ssubst{\svar{x}}{\sval}}
    {\sexpp\ssubst{\svar{x}}{\scoerce{\sarrow{\staui}{\stauii}}{\cdot}{\tval}}}$
\end{corollary}


==> interop_lazy/cortop.tex <==
\begin{corollary}[Top-level correctness statement]\ \\
  If
  \begin{itemize}
  \item $\hastyp{\cdot}{\cdot}{\sexp}{\ssig}$
  \item $\sexp \trans \texp$
  \end{itemize}
  then
  $\sexp \sctxeq \salien{\texp}{\ssig}{\cdot} $ for the standard notion of contextual equivalence.
\end{corollary}


==> interop_lazy/embed.tex <==
\[
\begin{array}{r l l}
  \kap{\stunit}{\sdelta}{\sexp}{k} & = & k ~ \tunit
  \\[0.3em]
  %
  \kap{\sarrow{\staui}{\stauii}}{\sdelta}{\sexp}{k} & = &
  k~\talien{\sexp}{\sarrow{\staui}{\stauii}}{\sdelta}
  \\[0.3em]
  %
  \kap{\sprod{\staui}{\stauii}}{\sdelta}{\sexp}{k} & = &
  \kap{\staui}{\sdelta}{\sfst{\sexp}}{\mfun{\texpi}{\kap{\stauii}{\sdelta}{\ssnd{\sexp}}{\mfun{\texpii}{k~\tpair{\texpi}{\texpii}}}}}
  \\[0.3em]
  \kap{\ssum{\staui}{\stauii}}{\sdelta}{\sexp}{k} & = &
  \scasex{e}
         {\sdelta\staui}{\kap{\staui}{\sdelta}{\svar{x}}{\mfun{\texp}{k~\tpar{\tinl{\texp}}}}}
         {\sdelta\stauii}{\kap{\stauii}{\sdelta}{\svar{x}}{\mfun{\texp}{k~\tpar{\tinr{\texp}}}}}
  \\[0.3em]
  \kap{\sall{\svar{A}}{\stau}}{\sdelta}{\sexp}{k} & = &
  k~\talien{\sexp}{\sall{\svar{A}}{\stau}}{\sdelta}
  \\[0.3em]
  \kap{\svar{A}}{\sdelta}{\sexp}{k} & = &
  k~\topaque{\sexp}
  \\[0.3em]
 %
 %% \\
 %% %
 %% \coerce{\ssum{\staui}{\stauii}}{\sdelta}{\sinl{\sexp}} & = &
 %% \tinl{\talien{\sexp}{\staui}{\sdelta}}
 %% \\
 %% %
 %% \coerce{\ssum{\staui}{\stauii}}{\sdelta}{\sinr{\sexp}} & = &
 %% \tinr{\talien{\sexp}{\stauii}{\sdelta}}
 %% \\
 %% %
 %% \coerce{\sall{\svar{A}}{\stau}}{\sdelta}{\stabs{\svar{A}}{\sexp}} & = &
 %% \talien{\sexp}{\stau}{\sesubstext{\sdelta}{\svar{A}}{\sttop}}
 %% \\
 %% %
 %% \coerce{\sttop}{\sdelta}{\salien{\tval}{\staup}{\sdeltap}} & = &
 %% \tval
 %% \\
\end{array}
\]


==> interop_lazy/fundamental.tex <==
\begin{theorem}[Correctness of the translation] \ \\

  For all $k \in \mathcal{N}$, if
  \begin{itemize}
  \item $\hastyp{\stenv}{\senv}{\sexp}{\stau}$
  \item $\sexp \trans \texp$
  \item $\inrtypenv{\delta}{\stenv}$
  \item $\inrenv {\sigma_1}{\sigma_2}{\senv}{k}$
  \end{itemize}
  then
  $\rexp{k}{\delta\sigma_1\sexp}
  {\salien{\delta\sigma_2\texp}{\stau}{\sdelta}}$
\end{theorem}


==> interop_lazy/log_rel.tex <==
\[
\begin{array}{r l l}
  \rval{k}{\salien{\texpi}{\staui}{\sdeltai}}{\salien{\texpii}{\stauii}{\sdeltaii}} & \defeq &
  \rtexp{k}{\texpi}{\texpii}
  \\[0.3em]
  %
  \rval{k}{\sunit}{\sunit} & \defeq & \top
  \\[0.3em]
  %
  \rval{k}{\spair{\sexpi}{\sexpii}}{\spair{\sexpip}{\sexpiip}}
  & \defeq &
  \rexp{k}{\sexpi}{\sexpip} \wedge  \rexp{k}{\sexpii}{\sexpiip}
  \\[0.3em]
  %
  \rval{k}{\sinl{\sexp}}{\sinl{\sexpp}}
  & \defeq &
  \rexp{k}{\sexp}{\sexpp}
  \\[0.3em]
  %
  \rval{k}{\sinr{\sexp}}{\sinr{\sexpp}}
  & \defeq &
  \rexp{k}{\sexp}{\sexpp}
  \\[0.3em]
  %
  \rval{k}{\sabs{\svar{x}}{\staui}{\sexpi}}{\sabs{\svar{y}}{\stauii}{\sexpii}}
  & \defeq &
  \forall (i < k)~\svali~\svalii, ~\rval{i}{\svali}{\svalii} \Rightarrow
  \rexp{i}{\sexpi\ssubst{\svar{x}}{\svali}}{\sexpii\ssubst{\svar{y}}{\svalii}}
  \\[0.3em]
  %
  \rval{k}{\stabs{\svar{A}}{\sexpi}}{\stabs{\svar{A}}{\sexpii}}
  & \defeq &
  \forall ~\staup, \iswf{}{\staup}  \Rightarrow
  \rexp{k}{\sexpi\ssubst{\svar{A}}{\staup}}{\sexpii\ssubst{\svar{A}}{\staup}}
  \\[0.3em]
  %
  & &   \\[0.3em]
  %
  & &   \\[0.3em]
  % 
  \rexp{k}{\sexpi}{\sexpii} & \defeq &
  \forall (m < k)~\svali,~ {\sexpi}\sevalm{m}{\svali} \wedge \isval{\svali} \Rightarrow \\[0.3em]
  & & ~~~~~~~~~~~~~~~~~~
  \exists~\svalii,~ {\sexpii}\sevals{\svalii} \wedge \rval{k - m}{\svali}{\svalii}
  \\[0.3em]
   %
  & &   \\[0.3em]
  %
  & &   \\[0.3em]
  % 
  \renv{\cdot}{k} & \defeq & \setsingl{(\cdot, \cdot )}  \\[0.3em]
  %
  \renv{\senvext{\senv}{\svar{x}}{\stau}}{k} & \defeq &
  \setst{(\sigma_1\sesubstsingl{\svar{x}}{\svali}}{\sigma_2\sesubstsingl{\svar{x}}{\svalii})}{\rval{k}{\svali}{\svalii}
  \wedge \inrenv{\sigma_1}{\sigma_2}{\senv}{k}}  \\[0.3em]
  %
  & &   \\[0.3em]
  %
  & &   \\[0.3em]
  % 
  \rtypenv{\cdot} & \defeq & \setsingl{\cdot}  \\[0.3em]
  %
  \rtypenv{\stenv,\svar{A}} & \defeq &
  \setsto{(\delta\sesubstsingl{\svar{A}}{\stau}}
  {\iswf{\stenv}{\stau}
  \wedge \inrtypenv{\delta}{\stenv}}  \\[0.3em]
\end{array}
\]


==> interop_lazy/trg_log_rel.tex <==
\[
\begin{array}{r l l}
  \rtval{k}{\topaque{\sexpi}}{\topaque{\sexpii}} & \defeq &
  \rexp{k}{\sexpi}{\sexpii}
  \\[0.3em]
  %
  \rtval{k}{\tunit}{\tunit} & \defeq & \top
  \\[0.3em]
  %
  \rtval{k}{\tpair{\texpi}{\texpii}}{\tpair{\texpip}{\texpiip}}
  & \defeq &
  \rtexp{k}{\texpi}{\texpip} \wedge  \rtexp{k}{\texpii}{\texpiip}
  \\[0.3em]
  %
  \rtval{k}{\tinl{\texp}}{\tinl{\texpp}}
  & \defeq &
  \rtexp{k}{\texp}{\texpp}
  \\[0.3em]
  %
  \rtval{k}{\tinr{\texp}}{\tinr{\texpp}}
  & \defeq &
  \rtexp{k}{\texp}{\texpp}
  \\[0.3em]
  %
  \rtval{k}{\tabs{\tvar{x}}{\texpi}}{\tabs{\tvar{y}}{\texpii}}
  & \defeq &
  \forall (i < k)~\tvali~\tvalii, ~\rtval{i}{\tvali}{\tvalii} \Rightarrow
  \rtexp{i}{\texpi\tsubst{\tvar{x}}{\tvali}}{\texpii\tsubst{\tvar{y}}{\tvalii}}
  \\[0.3em]
  %
  %% \rtval{k}{\stabs{\svar{A}}{\sexpi}}{\stabs{\svar{A}}{\sexpii}}
  %% & \defeq &
  %% \forall ~\stau', \iswf{}{\stau'}  \Rightarrow
  %% \rexp{k}{\sexpi\ssubst{\svar{A}}{\stau'}}{\sexpii\ssubst{\svar{A}}{\stau'}}
  %% \\[0.3em]
  %
  & &   \\[0.3em]
  %
  & &   \\[0.3em]
  % 
  \rtexp{k}{\texpi}{\texpii} & \defeq &
  \forall (m < k)~\tvali,~ {\texpi}\tevalm{m}{\tvali} \wedge \isval{\tvali} \Rightarrow \\[0.3em]
  & & ~~~~~~~~~~~~~~~~~~
  \exists~\tvalii,~ {\texpii}\tevals{\tvalii} \wedge \rtval{k - m}{\tvali}{\tvalii} 
  \\[0.3em]
   
  & &   \\[0.3em]
  %
  & &   \\[0.3em]
  % 
  \rtenv{\cdot}{k} & \defeq & \setsingl{(\cdot, \cdot )}  \\[0.3em]
  %
  \rtenv{\tenvext{\tenv}{\tvar{x}}}{k} & \defeq &
  \setst{(\sigma_1\tesubstsingl{\tvar{x}}{\tvali}}{\sigma_2\tesubstsingl{\tvar{x}}{\tvalii})}{\rtval{k}{\tvali}{\tvalii}
  \wedge \inrtenv{\sigma_1}{\sigma_2}{\tenv}{k}}  \\[0.3em]
  %% %
  %% & &   \\[0.3em]
  %% %
  %% & &   \\[0.3em]
  %% % 
  %% \rtenv{\cdot} & \defeq & \setsingl{\cdot}  \\[0.3em]
  %% %
  %% \rtenv{\Delta,\svar{A}} & \defeq &
  %% \setsto{(\delta\sesubstsingl{\svar{A}}{\stau}}
  %% {\iswf{\Delta}{\stau}
  %% \wedge \inrtenv{\delta}{\Delta}}  \\[0.3em]
\end{array}
\]


==> interop_lazy/trg_typing.tex <==
\begin{mathpar}
\inferrule*[right=Alien]
 {\hastyp{\stenv}{\senv}{\sexp}{\sesubst \stau}}
 {\isok{\stenv}{\senv}{\talien{\sexp}{\stau}{\sdelta}}}
  %
  \and
  %
  \inferrule*[right=Opaque]
  {\\}
  {\isok{\stenv}{\senv}{\topaque{\sexp}}}
  %
  \and
  %
  \inferrule*[right=Unit]
  {\\}
  {\isok{\stenv}{\senv}{\tunit}}
  %
  \and
  %
  \inferrule*[right=Pair]
  {\isok{\stenv}{\senv}{\texpi} \\
   \isok{\stenv}{\senv}{\texpii}}
  {\isok{\stenv}{\senv}{\tpair{\texpi}{\texpii}}}
  %
  \and
  %
  \inferrule*[right=Abs]
  {\isok{\stenv}{\senv}{\texp}}
  {\isok{\stenv}{\senv}{\tabs{\tvar{x}}{\texp}}}
 
  %% \inferrule*[right=Opaque]
  %% {\\}
  %% {\hastyp{\senv}{\sopaque{\texp}}{\sttop}}
\end{mathpar}


==> lstfstar.tex <==
\newcommand\function{\sffamily\maybecolor{dkblue}function}

\makeatletter
\lstdefinelanguage{fstar}{%
  basicstyle=\small,
  morekeywords=[1]{type,and,val,fun,let,in,ref,uref,mref,try,if,then,else,match,with,open,as,module,rec,begin,end,assume,private,when,forall,assert,by_tactic,logic,array,pattern,effect,requires,ensures,decreases,modifies, abstract,total, reifiable, reflectable, new, new_effect, effect_actions, noeq, sub_effect, by, synth,splice},
  morekeywords=[2]{WP, Post, Pre, Pure , PURE, DIV, STATE, EXN, ALL, TotST, M, GHOST, Ghost, GTot, Lemma, Tot, Div, DIV, Memo, READER, STATE_m, Effect, STEXN, RANDOM, ST, St, MST, S_MST, MSTExn, TAC, Tac, TacH},
  morekeywords=[3]{},
  morekeywords=[4]{},
  morestring=[b]",
  sensitive=true,%
  numbersep=4pt,
%  numbers=left,
  columns=[l]fullflexible,
  texcl=true,
  mathescape=true,
%  xleftmargin=10pt,
  identifierstyle={\sffamily},
  keywordstyle=[1]{\sffamily\maybecolor{dkblue}},
  keywordstyle=[2]{\sffamily\maybecolor{dkblue}},
  keywordstyle=[3]{\maybecolor{dkred}},
  keywordstyle=[4]{\rmfamily\itshape},
% Here is the range marker stuff
  rangeprefix=(*---\ ,
  includerangemarker=false,
  stringstyle=\ttfamily,
  %lineskip=-2pt,
  showspaces=false,
  morecomment=[n]{(*}{*)},
  commentstyle={\itshape\maybecolor{dkred}},
  literate={->}{$\rightarrow\,$}{1}
           {True}{$\top$}{1}
           {False}{$\bot$}{1}
           {exists}{$\exists$}{1}
           {forall}{$\forall$}{1}
           {fun}{$\lambda$}{1}
           {func}{func}{1}
           {~}{$\neg$}{1}           
           {~>}{$\leadsto$}{1}
           {`}{\`{}}{1}
           {'a}{$\alpha$}{1}
           {'b}{$\beta$}{1}
           {'c}{$\gamma$}{1}
           {phi}{$\phi\,$}{1}
           {tau}{$\tau\,$}{1}
           {tauto}{tauto}{6}
           {psi}{$\psi\,$}{1}
           {xi}{$\xi\,$}{1}
           {VC_e}{VC$_e$}{1}
           {Gamma}{$\Gamma\,$}{1}
           {theta}{$\theta\,$}{1}
           {_0}{$_0$}{1}
           {_1}{$_1$}{1}
           {_2}{$_2$}{1}
           {_3}{$_3$}{1}
           {_4}{$_4$}{1}
           {STATE0}{$\mathsf{ST}^\prime\,$}{1}
           {/\\}{$\wedge\;$}{1}
           {\\/}{$\vee\;$}{1}
           {>=}{$\geq\ $}{2}
           {<=}{$\leq\ $}{2}
           {<==>}{$\Longleftrightarrow \ $}{3}
           {==>}{$\Longrightarrow \ $}{3}
           {|->}{$\mapsto \ $}{3}
           {|>}{$\mapsto \ $}{2}
           %% {dot}{$\bullet \ $}{3}
           %% {nat}{$\mathbb{N}$}{3}
           %% {emp}{$\emptyset$}{3}
     {<>}{$\neq$}{1}
     {<*>}{$\bullet \ $}{3}
     {--}{-}{1}   % Added due to         - not displaying properly.  Weird. ... but may make arrows look bad  {...}{$\ldots$}{3}
     {<<}{$\prec\ $}{1}
           ,
  breaklines=false}
\makeatother


==> texdirectives.tex <==
\draftfalse\anonfalse\camerafalse\fulltrue

